Resilience Bounds of Sensing-Based Network Clock Synchronization

Recent studies exploited external periodic synchronous signals to synchronize a pair of network nodes to address a threat of delaying the communications between the nodes. However, the sensing-based synchronization may yield faults due to nonmalicious signal and sensor noises. This paper considers a system of N nodes that will fuse their peer-to-peer synchronization results to correct the faults. Our analysis gives the lower bound of the number of faults that the system can tolerate when N is up to 12. If the number of faults is no greater than the lower bound, the faults can be identified and corrected. We also prove that the system cannot tolerate more than N-2 faults. Our results can guide the design of resilient sensing-based clock synchronization systems.

==> backup.tex <==
\begin{comment}
\section{Decoding Fault Tolerant Scheme}

 Each CPS node derives its logical clock from a physical clock. This Physical clock may fail to maintain consistency with perfect clock. The rate at which the clock is deviating from perfect clock is called \textit{drift rate}. The rate at which each physical clock drifts with respect to one other is called \textit{clock skew}. 

 Consider a set of N nodes denoted by $\{n_1,n_2,...,n_N\}$. Clock offset between the nodes $n_i$ and $n_j$ is denoted as $\delta_{ij}$ that is unknown and to be estimated. Specifically, $\delta_{ij} = c_j(t) - c_i(t)$, wherein $c_i(t)$ and $c_j(t)$ are the clock values of $n_i$ and $n_j$ at any given time instant \textit{t}. To simplify the discussion, assume $\delta_{ij}$ as time-invariant. By designating $n_1$ as the reference node,$\delta_{ij}$ can be expressed as $\delta_{ij} = \delta_{1j} - \delta_{1i}$.

\begin{defn} (Reference Node). Reference node is a node whose sync-sessions with other N-1 nodes in the system is used to characterize the sync-sessions between each pair of N-1 nodes (excluding  reference node) that establishes sync-session with reference node. \end{defn}

In figure 1, nodes are represented as vertices and edges denotes sync-sessions. For a 3 node system, let node 1 be the reference node. Then, edges e12,e13,e23 represents the sync-session between the nodes 1\&2, 1\&3 and 2\&3 respectively. The sync-session e23 can be characterized using the sync-sessions e12 and e13.  

\begin{figure}
\centering
\includegraphics[width = 3cm,height=3cm]{eps/ex.jpg}
\caption{Example for reference node,layer-1 and layer-2 equations}
\end{figure}

If clock-sync error occurs between $n_i$ and $n_j$, it is denoted as $e_{ij}$. $\tilde {\delta}_{ij}$ denotes measured offset through clock synchronisation session between $n_i$ and $n_j$. Thus, when no synchronisation error occurs, $\tilde {\delta_{ij}}$ = $\delta_{ij}$; when synchronisation error occurs,$\tilde {\delta_{ij}}$ = $\delta_{ij} + e_{ij}$. $\hat {\delta}_{ij}$ and $\hat {e}_{ij}$ denotes estimates of $\delta_{ij}$ and $e_{ij}$ respectively. Number of actual and estimated errors are denoted as $Ka$ and $k$ respectively. 

 To determine the tolerance of a system, a set of linear equations representing sync-sessions is formed by equating estimate offsets \& errors with ground-truth offsets \& errors respectively. This system of equations is solved for estimate offset $\hat{\delta_{ij}}$ and estimate error $\hat{e}_{ij}$. $\hat{\delta_{ij}}$, $\hat{e}_{ij}$ is expected to obtain the corresponding ground-truth offset $\delta_{ij}$ and ground-truth error $e_{ij}$ as solution. These variables are chosen in order to find the corresponding counterpart. 

\begin{exmp} For a 3-node system represented in figure 1, in the presence of one ground-truth error and corresponding estimate error, the system of equations can be represented as follows.\\
$\hat{\delta}_{12} + \hat{e}_{12} = {\delta}_{12} + {e}_{12}$ \\
$\hat{\delta}_{13} = {\delta}_{13}$\\
$\hat{\delta}_{13} - \hat{\delta}_{12} = {\delta}_{13} - {\delta}_{12}$\end{exmp}

\begin{defn} (Layer-1 and Layer-2 equations) The equations representing the sync-sessions between Reference node and the other N-1 nodes are called as Layer-1 equations. The equations representing sync-sessions between each pair of N-1 nodes except reference node are called as Layer-2 equations. \end{defn}

 For a 3-node system represented in figure 1, the sync-sessions can be represented using equations are as given above with \textit{Node 1} as reference node. In those equations, first two equations belongs to Layer-1 group as it represents the sync-sessions between nodes 1\&2 and 1\&3. Last equation belongs to Layer-2 group as it represents the sync sessions between the nodes 2\&3.\\

\begin{defn} {Fault Tolerance for Clock-sync errors} To be written after discussion. \end{defn}

\textit{Algorithm 1} determines fault tolerance of clock-sync errors. It solves the following equation system for $\hat{\delta}_{ij}, e_{ij}$.\\
$\hat{\delta}_{1i} + \hat{e}_{1j}= \tilde{{\delta}}_{1j}$;  j $\epsilon$ $\{2,3,...N\}$\\
$\hat{\delta}_{1j} - \hat{\delta}_{1i} + \hat{e}_{1j} = \tilde{{\delta}}_{ij}; i,j \epsilon \{2,3,...N\}, i \neq j.$\\
To classify solutions, initially an augmented matrix $[A|B]$ is formed. $A$ is the coefficient matrix that holds chosen variables of equations (i.e) it holds $\hat{\delta}_{ij}, e_{ij}$ while $B$ holds the rest. Obtained solution is then classified based on the \textit{rank(A)} and \textit{rank([A$|$B])}.\\
 While solving, we expect $\hat{\delta}_{ij}$ , $e_{ij}$ to find the corresponding ${\delta}_{ij}$ and  $\hat{e}_{ij}$ respectively leading to an Unique \& Correct solution. Further classification of solution is described in \textit{Algorithm 2} based on Rouche-Capelli theorem\cite{Shafarevich2012}. Rouche-Capelli theorem is stated as. \\
\textit{
	A system of linear equations with n variables has a solution if and only if the rank of its coefficient matrix A is equal to the rank of its augmented matrix [A$|$B].If there are solutions, they form an affine subspace of  ${\displaystyle \mathbb {R} ^{n}}$ of dimension $n - rank(A)$.In particular:
	\begin{itemize}
		\item if n = rank(A), the solution is unique,
		\item otherwise there is an infinite number of solutions.
	\end{itemize}
}
\textit{Algorithm 1} determines whether the system is tolerant to clock-sync errors. Lines [5-10] stores measured and estimate offsets in \textit{X} and \textit{G} arrays respectively. Lines [11 - 17] stores estimate errors in array \textit{E}. Lines [18 - 20] \& lines [21 - 27] forms Layer 1 \& Layer 2 equations respectively and stores them in \textit{eqns} array. Lines [28-30] stores estimate offsets in \textit{vars} array. Lines [39 - 41] describes the way in which estimated errors are distributed to the formed equations and solved for variables stored in \textit{vars} array. IN lines [41 - 46], solution set is classified according to algorithm 2. If Unique \& Correct solution is found, \textit{sol} is returned.  

\begin{algorithm}
	\caption{Determining Tolerance of an N-Node system}
	\begin{algorithmic}[1]
	\State Input: Number of Nodes (N)
	\State Output: Tolerant or Intolerant
	\State R (reference node) = Node running this algorithm
	\State T = 1
	\For {i = 1 to N-1}
	\If {i $\neq$ R}
	\State X[i] = $\tilde{\delta}_{Ri}$ (Measured offsets)
	\State G[i] = $\hat{\delta}_{Ri}$ (Estimate offsets) 
	\EndIf
	\EndFor
	\For {i = 1 to N}
	\For {j = 1+1 to N}
	\If {i $\neq$ j}
	\State E[] = $e_{ij}$ (Estimate errors)
	\EndIf
	\EndFor
	\EndFor
	\For {i = 1 to N-1}
	\State eqns[i] = X[i] == G[i]
	\EndFor
	\For {j = N-1 to 1}
	\For {i = 1 to N-1}
	\If {i $\neq$ j}
	\State eqns[] = X[j] - X[i] == G[j] - G[i]
	\EndIf
	\EndFor
	\EndFor
	\For{ i = 0 to N-1}
	\State vars[i]  = G[i]
	\EndFor
	\For {i = 0 to N-3}
		\For {m = 1 to N(N-1)/2} 
			\For {n = 1 to size(L)}
				\If{eqns[m] != L[n]}
					\State eqns1[m] == eqns[m]
				\ElsIf{eqns[m] == L[n]}
					\State eqns1[m] = LHS(eqns[m]) == RHS(eqns[m]) + E[m]
					\State append E[m] to vars[]
				\EndIf
			\EndFor
		\EndFor
		\State sol = solve(eqns1,vars)
		\State Classify solutions according to \textit{Algorithm 2}
		\If {sol = Unique and correct}
			\State Return sol and break
		\EndIf
	\EndFor	
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{Classification of Solutions}
	\begin{algorithmic}[1]
		\State Input: rank(A); rank(A,B); Solutions obtained for $e_{ij}$ values; Expected Solution
		\State Output: Returns the type of Solution.
		\If{rank(A) $\neq$ rank(A,b)}
		\State Return No Solution
		\ElsIf{rank(A) $==$ rank[A$|$B]}
		\If{rank(A) $\neq$ number of variables}
		\State Return Infinitely Many Solutions
		\ElsIf{any $e_{ij}$ variable is 0}
		\State Return No Solution
		\Else
		\State Unique Solution
		\If{expected solution $==$ obtained solution}
		\State Return Unique\&Correct Solution 
		\Else
		\State Return Unique\&Wrong Solution
		\EndIf
		\EndIf
		\EndIf
	\end{algorithmic}
\end{algorithm}
\end{comment}


==> bounds.tex <==
\section{Bounds of Maximum Resilience}

\subsection{Lower Bound of Maximum Resilience}
\label{subsec:symbolic}

  \begin{lemma}
    $\mat{A}' \vec{x}' = \vec{b}'$ always has one or more solutions. When $\mat{A}'$ has full column rank, the original $\mat{A} \vec{x} = \vec{b}$ either has no solutions or has a unique correct solution.
    %; when $\mat{A}'$ is not full column ranked,
    \label{lem:1}
  \end{lemma}
  \begin{proof}
    The $\vec{x}'$ satisfying (i) $\hat{\delta}_{j0} = \delta_{j0}$, $\forall j \in [1, N-1]$, (ii) $\hat{\vec{e}} = \vec{0}$, and (iii) $\vec{e}=\vec{0}$ must be a solution. We denote this solution as $\vec{x}_0'$. As shown in previous examples, $\mat{A}'\vec{x}'=\vec{b}'$ can have an infinite number of solutions. Therefore, $\mathrm{rank}(\mat{A}' | \vec{b}') = \mathrm{rank}(\mat{A}')$ always holds and $\mat{A}'\vec{x}' = \vec{b}'$ always has one or more solutions.

    When $\mat{A}'$ has full column rank, $\mat{A}'\vec{x}'=\vec{b}'$ has a unique solution that must be $\vec{x}_0'$. The $\vec{e}=\vec{0}$ in this solution means that the original $\mat{A}\vec{x} = \vec{b}$ does not allow any p2p synchronization error. We now consider two cases. First, in the presence of any p2p synchronization error, the $\mat{A}\vec{x} = \vec{b}$ must have no solutions; otherwise, the solution of $\mat{A}\vec{x} = \vec{b}$ conflicts with the unique solution of $\vec{A}'\vec{x}'=\vec{b}'$ with $\vec{e}=\vec{0}$. Second, in the absence of synchronization error, the unique solution $\vec{x}_0'$ encompasses the unique correct solution of $\mat{A}\vec{x}=\vec{b}$.
%    In other words, in the presence of any p2p synchronization error, the $\mat{A}\vec{x} = \vec{b}$ must have no solutions; in the absence of p2p synchronization error,
  \end{proof}
  
  The following proposition is a tool to find the lower bound of maximum resilience.
  
  \begin{proposition}
    A system is $K$-resilient if $\forall k \in [0, K]$, for any distribution of the $K$ actual p2p synchronization errors and any distribution of the $k$ estimated p2p synchronization errors, $\mat{A}'$ has full column rank.
  \end{proposition}

  \begin{proof}
    From Lemma~\ref{lem:1}, as $\mat{A}'$ has full column rank, the original $\mat{A}\vec{x}=\vec{b}$ either has no solutions or has a unique correct solution. We now analyze the cases considered in Definition~\ref{def:resilience-condition}:
    \begin{enumerate}
    \item when $k \in [0, K)$, since $k < K$, the solution of $\mat{A}\vec{x}=\vec{b}$ cannot be correct. Thus, the $\mat{A}\vec{x}=\vec{b}$ has no solutions.
    \item when $k=K$,
      \begin{enumerate}
      \item if the distribution of the $k$ estimated p2p synchronization errors is identical to the actual distribution, as the statement that $\mat{A}\vec{x}=\vec{b}$ has no solution must not be true (because the correct solution is a solution), $\mat{A}\vec{x}=\vec{b}$ must have a unique (and correct) solution.
      \item otherwise, since the distributions are different, the solution of $\mat{A}\vec{x}=\vec{b}$ cannot be correct. Thus, the $\mat{A}\vec{x}=\vec{b}$ has no solutions.
      \end{enumerate}
    \end{enumerate}
    In summary, a full column rank $\mat{A}'$ ensures that the $K$-resilience condition is satisfied.
  \end{proof}

\subsection{Upper Bounds of Maximum Resilience}
\label{subsec:upper-bounds}

\begin{proposition}
  An $N$-node system is not $K$-resilient when $K \ge N-1$.
\end{proposition}

\begin{table*}
  \normalsize
  \begin{minipage}{\textwidth}
    \begin{equation}
      \mat{A} = 
      \begin{blockarray}{ccccccccc}
        &\hat{\delta}_{10}& \cdots &\hat{\delta}_{(N-1)0}&\hat{e}_{10}& \hat{e}_{12} & \cdots & \hat{e}_{1(N-1)} & \cdots \\
        \begin{block}{c(cccccccc)}
          n_0 \leftrightarrow n_1       &1                & \cdots                & \cdot                &1           & 0 & \cdots  & 0 & \cdots \\
          n_0 \leftrightarrow n_2       &0                & \cdots                & \cdot                &0           & 0  & \cdots & 0 & \cdots \\
          n_i \leftrightarrow n_j, \forall i,j \neq 1        & \vdots                 & \ddots                & \vdots                & \vdots           & \vdots & \ddots & \vdots & \ddots \\
          n_{N-2} \leftrightarrow n_{N-1}       &0                &\cdots                & \cdot                &0           & 0 & \cdots & 0 & \cdots \\
          n_1 \leftrightarrow n_2       & -1                & \cdots                & \cdot                &0           & 1 & \cdots & 0 & \cdots \\
          \vdots        & \vdots                 & \ddots                & \vdots                & \vdots           & \vdots  & \ddots & \vdots & \ddots \\
          n_1 \leftrightarrow n_{N-1}       & -1                & \cdots                & \cdot                &0           & 0 & \cdots & 1 & \cdots \\
        \end{block}
      \end{blockarray}
      \label{eq:prop1}
    \end{equation}
    %\medskip
    \hrule
  \end{minipage}
\end{table*}

\begin{proof}
  We prove by an counterexample where all the $N-1$ p2p synchronization sessions involving the node $n_1$ are faulty. The remaining $K - (N - 1)$ faulty p2p synchronization sessions may occur between any other node pairs. Consider that Algorithm~\ref{alg:error-correction} is testing a distribution of the $K$ p2p synchronization errors that is identical to the actual distribution. Since the true clock offsets and the true p2p synchronization errors must form a valid solution to the equation system, we have $\mathrm{rank}(\mat{A} | \vec{b}) = \mathrm{rank}(\mat{A})$.

The matrix $\mat{A}$ of the vectorized equation system is given by Eq.~(\ref{eq:prop1}). We add labels to help understanding each column's corresponding unknown to be solved and each row's corresponding p2p synchronization session. In the first column of $\mat{A}$ that corresponds to the clock offset estimate $\hat{\delta}_{10}$, the first element and the last $N-2$ elements that correspond to all p2p synchronization sessions involving $n_1$ are non-zeros; all other elements are zero. This column is a linear combination of the columns corresponding to $\hat{e}_{10}, \hat{e}_{12}, \ldots, \hat{e}_{1(N-1)}$. Thus, $\mat{A}$ is not full column ranked. Therefore, the equation system $\mat{A}\vec{x} = \vec{b}$ have an infinite number of solutions, which violates the resilience condition.
\end{proof}


\begin{proposition}
  An $N$-node system is not $K$-resilient when $K \ge N-2$.
\end{proposition}

==> discuss.tex <==
\section{Discussions}
\label{sec:discuss}

definition of fault, and difference from fault and attack

%centralized vs decentralized. scalability. good network structure under a centralized scheme

%if the pair-wise sync is not feasible

%how to leverage the integer multiple property

%tight bound


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> eps/sensing.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4896.00,1764.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(507,1212){\makebox(0,0)[l]{\strut{}$T$}}%
      \put(441,17){\makebox(0,0)[l]{\strut{}$\phi_1$}}%
      \put(3095,17){\makebox(0,0)[l]{\strut{}$\phi_4$}}%
      \put(1768,1994){\makebox(0,0)[l]{\strut{}$\phi_2$}}%
      \put(2564,1994){\makebox(0,0)[l]{\strut{}$\phi_3$}}%
      \put(883,1088){\makebox(0,0)[l]{\strut{}\texttt{request}}}%
      \put(2453,1088){\makebox(0,0)[l]{\strut{}\texttt{reply}}}%
      \put(4355,1624){\makebox(0,0)[l]{\strut{}$B$'s clock}}%
      \put(4355,388){\makebox(0,0)[l]{\strut{}$A$'s clock}}%
      \put(3869,-228){\makebox(0,0)[l]{\strut{}Newtonian time}}%
      \put(595,388){\makebox(0,0)[l]{\strut{}$t_1$}}%
      \put(1967,1376){\makebox(0,0)[l]{\strut{}$t_2$}}%
      \put(2652,1376){\makebox(0,0)[l]{\strut{}$t_3$}}%
      \put(3426,182){\makebox(0,0)[l]{\strut{}$t_4$}}%
      \put(330,758){\makebox(0,0)[l]{\strut{}LI}}%
      \put(1502,1953){\makebox(0,0)[l]{\strut{}LI}}%
      \put(2387,1953){\makebox(0,0)[l]{\strut{}LI}}%
      \put(2851,758){\makebox(0,0)[l]{\strut{}LI}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{sensing}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> full.tex <==
\section{Error Correction Capability}


%\begin{small}
%
%\begin{theorem} A fully-connected \textit{N}-node system can correct a maximum of \textit{N-3} clock synchronisation errors. \end{theorem}
%
%\begin{defn} (Layer-1 and Layer-2 equations) The equations representing the sync-sessions between Reference node and the other N-1 nodes are called as Layer-1 equations. The equations representing sync-sessions between each pair of N-1 nodes except reference node are called as Layer-2 equations.\end{defn}
%
%The system of equations represent synchronisation sessions between each pair of nodes in a fully connected system. Hence, total number of equations will be $L$ = \textit{N(N-1)/2}. Out of these equations, \textit{N-1} is the number of Layer-1 equations and the rest are Layer-2 equations. There can be a maximum of \textit{N(N-1)/2} clock-sync errors. If \textit{N-3} number of clock-sync errors are present in the system, say \textit{M} of them are in Layer-1 equations. Here, \{ $\delta_1$,...,$\delta_{N-1}$\} represents \{ $\delta_{ij}$ $|$ $\forall$ i,j $\epsilon$ [0 , N-1], i $\neq$ j \} to make the system more generic so that this equation system can suit any number of Nodes N. This also suits to estimate offset $\hat{\delta}_{ij}$. Errors \{$e_1$,..,$e_{K}$\} represents \{$e_{ij}$ $|$ $\forall$ i,j $\epsilon$ [0 , N-1], i $\neq$ j \} to make the system generic. This also holds for estimate errors $\hat{e}_{ij}$. Given below is the generic structure of equation system without any errors.\\
%$\hat{\delta}_1 = {\delta}_1\\$
%$\hat{\delta}_2 = {\delta}_2\\$
%.\\
%.\\
%$\hat{\delta}_{N-1-M} = \delta_{N-1-M}$\\
%$\hat{\delta}_{N-M} = \delta_{N-M}$\\
%.\\
%.\\
%$\hat{\delta}_{N-2} = \delta_{N-2}$\\
%$\hat{\delta}_{N-1} = \delta_{N-1}$\\
%$\hat{\delta}_2 - \hat{\delta}_1 = \delta_2 - \delta_{1}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_1 = \delta_{N-1} - \delta_{1}\\$
%$\hat{\delta}_{N-M} - \hat{\delta}_{N-1-M} = \delta_{N-M} - \delta_{N-1-M}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_{N-2} = \delta_{N-1} - \delta_{N-2}\\ $
%
% Generic augmented matrix [A$|$ $\mathbf{b}$] for the above equation system is given below. \textit{A} holds the chosen variables $\hat{\delta}_{ij}$, $\hat{e}_{ij}$ while \textit{B} holds remaining variables of the equation. Rows are identified with row numbers represented under the column \textit{Row}. In the below matrix if errors are present in Layer-1 equations, it can appear only in rows $A_{N-M}$ to $A_{N-1}$ according to the assumption that Layer-1 equations contain \textit{M} errors. Similarly, If actual errors are present in Layer- 2 equations, it appears from $A_N$ to $A_{2N-4-M}$. If errors are arranged complying this generic structure,it can hold a maximum of \textit{N-3} errors.
%
%Generic matrix notation considering [$\hat{\delta}_{ij},\hat{e}_{ij}$] as variables can be represented as\\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1   &\cdots&\hat{e}_A&\cdots&\hat{e}_{K} &B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   &\cdots&  0      &\cdots&   0  &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0  &\cdots& 0       &\cdots& 0    &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots   &\vdots&\vdots&\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  &\cdots& 0       &\cdots& 0    &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   0  &\cdots& 0       &\cdots& 0    &{\delta}_{N-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots&\cdots&\vdots   &\vdots&\vdots&\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  &\cdots& 0       &\cdots& 0    &{\delta}_{N-2}\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0  &\cdots& 0       &\cdots& 0    &{\delta}_{N-1}\\
%	A_{N}     &-1            &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0   &\cdots& 0       &\cdots& 0    &{\delta}_2 - {\delta}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots   &\vdots&\vdots&\vdots\\
%	A_{2N-4-M}&-1            &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0   &\cdots& 0       &\cdots& 0    &{\delta}_{N-1}-{\delta}_1\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        -1          &     1            &\cdots&  0               &   0              &  0   &\cdots& 0       &\cdots& 0    &{\delta}_{N-M}-{\delta}_{N-1-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots   &\vdots&\vdots&\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& -1               &   1              &  0   &\cdots& 0       &\cdots& 0    &{\delta}_{N-1} - {\delta}_{N-2}\\
%	\end{block}
%	\end{blockarray}
%	$
%\end{scriptsize}
%
%\begin{lemma} \textit{N}-node system yields Unique\&Correct solution if $K \leq N-3$ actual errors and $k = K$ estimate errors are on the same sync-session equations.\end{lemma}
%
%\begin{proof} Consider an \textit{N}-node system containing $K \leq N-3$  actual and $k = K$ estimate errors such that actual and corresponding estimate errors are in the same sync-session equations. Then the generic equations can be modified as\\
%$\hat{\delta}_1 = {\delta}_1\\$
%$\hat{\delta}_2 = {\delta}_2\\$
%.\\
%.\\
%$\hat{\delta}_{N-1-M} = \delta_{N-1-M}$\\
%$\hat{\delta}_{N-M} + \hat{e}_1 = \delta_{N-M} + {e}_1$\\
%.\\
%.\\
%$\hat{\delta}_{N-2}  + \hat{e}_A = \delta_{N-2} + e_A$\\
%$\hat{\delta}_{N-1} = \delta_{N-1}$\\
%$\hat{\delta}_2 - \hat{\delta}_1 + \hat{e}_{k} = \delta_2 - \delta_{1} + e_{K} \\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_1 = \delta_{N-1} - \delta_{1}\\$
%$\hat{\delta}_{N-M} - \hat{\delta}_{N-1-M} = \delta_{N-M} - \delta_{N-1-M}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_{N-2} = \delta_{N-1} - \delta_{N-2}\\ $
%
%Modified generic matrix structure can be represented as\\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\cdots&\hat{e}_{K}&B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0      &\cdots&  0      &\cdots&   0        &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1     &\cdots& 0       &\cdots& 0          &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0     &\cdots&  1      &\cdots& 0          &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-1}\\
%	A_{N}     &-1            &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 1          &{\delta}_2-{\delta}_1+{e}_{K}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{2N-4-M}&-1            &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-1}-{\delta}_1\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        -1          &     1            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-M}-{\delta}_{N-1-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& -1               &   1              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-1} - {\delta}_{N-2}\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_N \rightarrow A_N + A_1\\
%A_{2N-4-M} \rightarrow A_{2N-4-M} + A_{1}\\
%A_{2N-3-M} \rightarrow A_{2N-3-M} + A_{N-1-M}\\
%A_L \rightarrow A_{N-2} + A_L \\$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW           &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1   &\cdots&\hat{e}_A&\cdots&\hat{e}_K &B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1           &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0         &\cdots&  0      &\cdots&   0      &{\delta}_1\\
%	A_2           &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0        &\cdots& 0       &\cdots& 0        &{\delta}_2\\
%	\vdots        & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots      &\cdots&\vdots   &\vdots&\vdots	&\vdots\\
%	A_{N-1-M}     &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0        &\cdots& 0       &\cdots& 0    	&{\delta}_{N-1-M}\\
%	A_{N-M}       &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1        &\cdots& 0       &\cdots& 0    	&{\delta}_{N-M} + {e}_1\\
%	\vdots        & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots      &\ddots&\vdots   &\vdots&\vdots	&\vdots\\
%	A_{N-2}       &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0        &\cdots&  1      &\cdots& 0    	&{\delta}_{N-2} + {e}_A\\
%	A_{N-1}       &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0        &\cdots& 0       &\cdots& 0    	&{\delta}_{N-1}\\
%	A_{N}         &0             &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0         &\cdots& 0       &\cdots& 1    	&{\delta}_2+{e}_{K}\\
%	\vdots        & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots      &\cdots&\vdots   &\vdots&\vdots	&\vdots\\
%	A_{2N-4-M}    & 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0         &\cdots& 0       &\cdots& 0    	&{\delta}_{N-1}\\
%	A_{2N-3-M}    & 0            &    0         &\cdots&        0           &     1            &\cdots&  0               &   0              &  0         &\cdots& 0       &\cdots& 0    	&{\delta}_{N-M}\\
%	\vdots        & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots      &\cdots&\vdots   &\vdots&\vdots	&\vdots\\
%	A_{L}         &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   1              &  0         &\cdots& 1       &\cdots& 0        &{\delta}_{N-1} + {e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_N \rightarrow A_N - A_2 \\
%A_{2N-4-M} \rightarrow A_{N-1} - A_{2N-4-M}\\
%A_{2N-3-M} \rightarrow A_{N-M} - A_{2N-3-M}\\
%A_L \rightarrow A_L - A_{N-1} \\$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\cdots&\hat{e}_K &B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   &\cdots&  0   &\cdots&   0  &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots&\vdots&\vdots&\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1  &\cdots& 0    &\cdots& 0    &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots&\ddots&\vdots&\vdots&\vdots&\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  &\cdots&  1   &\cdots& 0    &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_{N-1}\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0   &\cdots& 0    &\cdots&  1   &{e}_{K}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots&\vdots&\vdots&\vdots\\
%	A_{2N-4-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0   &\cdots& 0    &\cdots& 0    &0\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  1   &\cdots& 0    &\cdots& 0    & {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots&\vdots&\vdots&\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   0              &  0   &\cdots& 1    &\cdots& 0    &{e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_{N - M} \rightarrow A_{N-M} - A_{2N-3-M} \\
%A_{N-2} \rightarrow A_{N-2} - A_{L}\\
%A_{2N-4-M} \leftrightarrow A_{2N-3-M}\\
%A_{2N-4-M} \leftrightarrow A_L \\
%A_N \leftrightarrow A_{2N-3-M}$\\
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW           &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1   &\cdots&\hat{e}_A   &\cdots&\hat{e}_{K}  &B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   &\cdots&  0   &\cdots&   0  &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots&\vdots&\vdots&\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &  0   &\cdots& 0    &\cdots& 0    &{\delta}_{N-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots&\ddots&\vdots&\vdots&\vdots&\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_{N-2} \\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0  &\cdots& 0    &\cdots& 0    &{\delta}_{N-1}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\cdots&\vdots&\vdots&\vdots&\vdots\\
%	A_{2N-4-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0   &\cdots& 0    &\cdots& 0    &0\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &   1  &\cdots& 0    &\cdots& 0    &{e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots&\ddots&\vdots&\vdots&\vdots&\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   0              &  0   &\cdots&  1   &\cdots& 0    &{e}_A\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0   &\cdots& 0    &\cdots&  1   &{e}_{K}\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%From the above matrix structure obtained after row transformations of initial matrix, we can deduce that\\
%rank(A) = rank(A,B) = (N-1) + (N-3) = Number of variables. Also, the variables solved yields the corresponding counterpart to show Unique \& Correct solution.\\
%
%Without Loss of Generality, if $K \leq N-3$ actual and $k = K$ estimate errors are on the same sync-session equations, Unique\&Correct solution can be obtained. Hence, system is capable of correcting decoding errors if Unique\&Correct solution can be obtained while actual and estimate errors are on the same sync-session equations.\\  
%\end{proof}
%
%Refer Example III.1 for an illustration.
%
%\begin{lemma} \textit{N}-node system yields No Solution if $K \leq N-3$ errors are present such that actual and estimate errors are on different sync-session equations with \textit{k} = \textit{K}.\end{lemma}
%
%\begin{proof} Consider an \textit{N}-node system containing $K \leq N-3$ actual and  $k = K$ estimate errors such that actual and corresponding estimate errors are on different sync-session equations. There will be at-least one actual error hanging without the corresponding estimate error. Then the generic equations can be modified as\\
%$\hat{\delta}_1 = {\delta}_1\\$
%$\hat{\delta}_2 = {\delta}_2\\$
%.\\
%.\\
%$\hat{\delta}_{N-1-M} = \delta_{N-1-M}$\\
%$\hat{\delta}_{N-M} + \hat{e}_1 = \delta_{N-M} + e_1 $\\
%.\\
%.\\
%$\hat{\delta}_{N-2} + \hat{e}_A  = \delta_{N-2} + e_A$\\
%$\hat{\delta}_{N-1} + \hat{e}_{K} = \delta_{N-1}$\\
%$\hat{\delta}_2 - \hat{\delta}_1 = \delta_2 - \delta_{1} + e_{K}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_1 = \delta_{N-1} - \delta_{1}\\$
%$\hat{\delta}_{N-M} - \hat{\delta}_{N-1-M} = \delta_{N-M} - \delta_{N-1-M}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_{N-2} = \delta_{N-1} - \delta_{N-2}\\ $
%
%Modified generic matrix structure can be represented as\\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\cdots&\hat{e}_{K}&B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0      &\cdots&  0      &\cdots&   0        &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1     &\cdots& 0       &\cdots& 0          &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0     &\cdots& 1       &\cdots& 0          &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0  	  &\cdots& 0       &\cdots& 1          &{\delta}_{N-1}\\
%	A_{N}     &-1            &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_2 - {\delta}_1 + {e}_{K}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{2N-4-M}&-1            &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-1}-{\delta}_1\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        -1          &     1            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-M}-{\delta}_{N-1-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& -1               &   1              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-1} - {\delta}_{N-2}\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_N \rightarrow A_N + A_1\\
%A_{2N-4-M} \rightarrow A_{2N-4-M} + A_{1}\\
%A_{2N-3-M} \rightarrow A_{2N-3-M} + A_{N-1-M}\\
%A_L \rightarrow A_{N-2} + A_L \\$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\cdots&\hat{e}_{K}&B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0      &\cdots&  0      &\cdots&   0        &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1     &\cdots& 0       &\cdots& 0          &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0     &\cdots& 1       &\cdots& 0          &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &\cdots& 1          &{\delta}_{N-1}\\
%	A_{N}     &0             &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_2 + {e}_{K}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-1}\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     1            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{\delta}_{N-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   1              &  0      &\cdots& 1       &\cdots& 0          &{\delta}_{N-1} + {e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_N \rightarrow A_N - A_2 \\
%A_{2N-4-M} \rightarrow A_{N-1} - A_{2N-4-M}\\
%A_{2N-3-M} \rightarrow A_{N-M} - A_{2N-3-M}\\
%A_L \rightarrow A_{N-1} - A_L \\$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\cdots&\hat{e}_{K}&B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0      &\cdots&  0      &\cdots&   0        &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1     &\cdots& 0       &\cdots& 0          &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0     &\cdots& 1       &\cdots& 0          &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &\cdots& 1          &{\delta}_{N-1}\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{e}_{K}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 1          &0\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  1      &\cdots& 0       &\cdots& 0          &{e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   0              &  0      &\cdots& 1       &\cdots& -1         &{e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$A_{N - M} \rightarrow A_{N-M}  - A_{2N-3-M} \\
%A_{N-2} \rightarrow A_{N-2} - A_{L}\\
%A_{N-1} \rightarrow A_{N-1} + A_{L}\\
%A_N \leftrightarrow A_{2N-3-M}\\
%A_L \leftrightarrow A_{2N-4-M}\\
%A_N \leftrightarrow A_{2N-4-M}$ \\
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{ccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\cdots&\hat{e}_{K}&B\\
%	\begin{block}{c[ccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0      &\cdots&  0      &\cdots&   0        &{\delta}_1\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0    	   &{\delta}_2\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   0     &\cdots& 0       &\cdots& 0          &{\delta}_{N-M} \\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0     &\cdots& 0       &\cdots& 1          &{\delta}_{N-2}\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 1       &\cdots& 0          &{\delta}_{N-1} + {e}_A\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &    0             &\cdots&  0               &   0              &  1      &\cdots& 0       &\cdots& 0          &{e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   0              &  0      &\cdots& 1       &\cdots& 1          &{e}_A\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 1          &0\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\vdots&\vdots      &\vdots\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &\cdots& 0          &{e}_{K}\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%From the above matrix structure after row transformations of initial matrix, we can deduce that\\
%rank(A) $\neq$ rank(A,B) shows that No solution is obtained if $K \leq N-3$ actual errors and $k = K$ estimate errors are on different sync-session equations.\\
%
%WLOG, if $K \leq N-3$ actual and $k = K$ estimate errors are on different sync-session equations, No solution can be obtained. Hence, system is capable of correcting decoding errors if  No solution can be obtained for $K \leq N-3$ while actual and estimate errors are on different sync-session equations.\\ 
%\end{proof}
%For example, consider a 4-node system with K $\leq$ N-3 actual errors, k = K estimate errors such that actual and corresponding estimate errors are on different sync-sessions. The equation system can be represented as,\\
%
%$
%\hat{\delta}_{01} = \delta_{01} \\
%\hat{\delta}_{02} + \hat{e}_{02}= \delta_{02}\\
%\hat{\delta}_{03} = \delta_{03} + e_{03} \\
%\hat{\delta}_{02} - \hat{\delta}_{01} = \delta_{02} - \delta_{01}\\
%\hat{\delta}_{03} - \hat{\delta}_{01} = \delta_{03} - \delta_{01}\\
%\hat{\delta}_{03} - \hat{\delta}_{02} = \delta_{03} - \delta_{02}\\
%$
%
%Matrix for the above equation system can be written as\\
%
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{02}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0     		 &\delta_{01}\\
%	A_2       &0                &1                &0                &1     		 &\delta_{02} \\
%	A_3       &0                &0                &1                &0    		 &\delta_{03} + {e}_{03} \\
%	A_4       &-1               &1                &0                &0     		 &\delta_{02} - \delta_{01}\\
%	A_5       &-1               &0                &1                &0     		 &\delta_{03} - \delta_{01}\\
%	A_6       &0                &-1               &1                &0     		 &\delta_{03} - \delta_{02}\\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%On doing the following transformations matrix becomes,\\
%$
%A_4 \rightarrow A_4 + A_1 \\
%A_5 \rightarrow A_5 + A_1 \\
%A_6 \rightarrow A_6 + A_2 \\
%$
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{02}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0           &\delta_{01}\\
%	A_2       &0                &1                &0                &1     		 &\delta_{02} \\
%	A_3       &0                &0                &1                &0    		 &\delta_{03} + \hat{e}_{03} \\
%	A_4       &0                &1                &0                &0     		 &\delta_{02}\\
%	A_5       &0                &0                &1                &0     		 &\delta_{03}\\
%	A_6       &0                &0                &1                &1    		 &\delta_{03} \\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%On doing the following transformations matrix becomes,\\
%$
%A_4 \rightarrow A_2 - A_4\\
%A_5 \rightarrow A_5 - A_3\\
%A_6 \rightarrow A_6 - A_3\\
%$
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{02}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0           &\delta_{01}\\
%	A_2       &0                &1                &0                &1           &\delta_{02} \\
%	A_3       &0                &0                &1                &0           &\delta_{03} + {e}_{03}\\
%	A_4       &0                &0                &0                &1           &0\\
%	A_5       &0                &0                &0                &1           &{e}_{03}\\
%	A_6       &0                &0                &0                & 1          &-{e}_{03}\\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%On doing the following transformations matrix becomes,
%$
%A_2 \rightarrow A_2 - A_4\\
%A_5 \rightarrow A_5 - A_4\\
%A_6 \leftrightarrow A_4\\
%$
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{02}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0     &\delta_{01}\\
%	A_2       &0                &1                &0                &0     &\delta_{02} \\
%	A_3       &0                &0                &1                &0     &\delta_{03} + e_{03}\\
%	A_4       &0                &0                &0                &1     &-e_{03}\\
%	A_5       &0                &0                &0                &0     &e_{03}\\
%	A_6       &0                &0                &0                & 1    &0\\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%
%From the above matrix we can see that rank(A) $\neq$ rank(A,B) indicating that system yields No solution making the system capable of correcting decoding errors. \\
%\begin{corollary} N-node system yields No solution if $K \leq N-3$ with $k \leq K$. 
%
%If $k \leq K$, there will be at-least one equation with a lone actual error hanging without corresponding estimate error in the equation. This can be reduced to \textit{Lemma 3} condition yielding No solution.\\
%
%Without Loss of Generality, if $K \leq N-3$ with $k \leq K$ estimate errors, No solution can be obtained. Hence, system is capable of correcting decoding errors if  No solution can be obtained for an N-node system with $K \leq N-3$.\\
%\end{corollary}
%
%\begin{lemma} 
%\textit{N}-node system yields Unique and Correct solution while \textit{K} $>$ \textit{N-3} actual errors with \textit{k} $\leq$ \textit{K} if actual and estimate errors are on same equations equations.\end{lemma}
%\begin{proof}
%	This condition can be reduced to \textit{Lemma I.2} yeilding Unique and Correct Solution.
%\end{proof}
%
%\begin{lemma} \textit{N}-node system yields Unique and Wrong solution while \textit{K} $>$ \textit{N-3} actual errors with \textit{k} $\leq$ \textit{K} if actual and estimate errors are on different equations.\end{lemma}
%
%\begin{proof} A system that is not capable of correcting decoding errors, it has to yield Unique \& Wrong solution or Infinitely Many Solutions. Consider an \textit{N}-node system with \textit{K} $>$ \textit{N-3} actual errors and \textit{k} $\le$ \textit{K} estimate errors on different sync-session equations. Then, the generic structure of the equation system can be modified as\\
%$\hat{\delta}_1  + \hat{e}_{K+1} = {\delta}_1\\$
%$\hat{\delta}_2 = {\delta}_2 + e_{K+1}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1-M} = \delta_{N-1-M}$\\
%$\hat{\delta}_{N-M} + \hat{e}_{1} = \delta_{N-M} + {e}_{1}$\\
%.\\
%.\\
%$\hat{\delta}_{N-2} + \hat{e}_A = \delta_{N-2} + {e}_{A}$\\
%$\hat{\delta}_{N-1} + \hat{e}_B = \delta_{N-1} + {e}_{B}$\\
%$\hat{\delta}_2 - \hat{\delta}_1 + \hat{e}_C = \delta_2 - \delta_{1} + {e}_{C}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_1 + \hat{e}_{K} = \delta_{N-1} - \delta_{1} + {e}_{K}\\$
%$\hat{\delta}_{N-M} - \hat{\delta}_{N-1-M} = \delta_{N-M} - \delta_{N-1-M}\\$
%.\\
%.\\
%$\hat{\delta}_{N-1} - \hat{\delta}_{N-2} = \delta_{N-1} - \delta_{N-2}\\ $   
%
%Modified generic matrix structure can be represented as\\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\hat{e}_B&\hat{e}_C&\cdots&\hat{e}_{K}&\hat{e}_{K+1}&B\\
%	\begin{block}{c[cccccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   	  &\cdots&  0      &   0     &   0     &\cdots&   0        & 1            &{\delta}_1 \\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta_2} + {e}_{K+1}\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots 	  	  &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  	  &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1  	  &\cdots&0        &   0     &   0     &\cdots& 0          &     0        &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots	  &\ddots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  	  &\cdots& 1       &  0      & 0       &\cdots& 0          &  0           &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &  1      &   0     &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_B\\
%	A_{N}     &-1            &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   0     &  1      &\cdots& 0          &     0        &{\delta}_2 - {\delta}_1 + {e}_C\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{2N-4-M}&-1            &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0      &\cdots& 0       &   0     & 0       &\cdots&  1         &     0        &{\delta}_{N-1}-{\delta}_1 + {e}_{K}\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        -1          &     1            &\cdots&  0               &   0              &  0      &\cdots& 0       &    0    &  0      &\cdots& 0          &     0        &{\delta}_{N-M}-{\delta}_{N-1-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots	  &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& -1               &   1              &  0   	  &\cdots& 0       &    0    &  0      &\cdots& 0          &     0        &{\delta}_{N-1} - {\delta}_{N-2}\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_N \rightarrow A_N + A_1\\
%A_{2N-4-M} \rightarrow A_{2N-4-M} + A_{1}\\
%A_{2N-3-M} \rightarrow A_{2N-3-M} + A_{N-1-M}\\
%A_L \rightarrow A_{N-2} + A_L \\$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\hat{e}_B&\hat{e}_C&\cdots&\hat{e}_{K}&\hat{e}_{K+1}&B\\
%	\begin{block}{c[cccccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   	  &\cdots&  0      &   0     &   0     &\cdots&   0        & 1            &{\delta}_1 \\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta_2} + {e}_{K+1}\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots 	  	  &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  	  &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1  	  &\cdots&0        &   0     &   0     &\cdots& 0          &     0        &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots	  &\ddots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  	  &\cdots& 1       &  0      & 0       &\cdots& 0          &  0           &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &  1      &   0     &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_B\\
%	A_{N}     &0             &    1         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   0     &  1      &\cdots& 0          &     1        &{\delta}_2 + {e}_C\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   1              &  0      &\cdots& 0       &   0     & 0       &\cdots&  1         &     1        &{\delta}_{N-1}+ {e}_{K}\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     1            &\cdots&  0               &   0              &  0      &\cdots& 0       &    0    &  0      &\cdots& 0          &     0        &{\delta}_{N-M}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots	  &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   1              &  0   	  &\cdots& 1       &    0    &  0      &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_N \rightarrow A_2 - A_N \\
%A_{2N-4-M} \rightarrow A_{2N-4-M} - A_{N-1}\\
%A_{2N-3-M} \rightarrow A_{N-M} - A_{2N-3-M}\\
%A_L \rightarrow A_L - A_{N-1} \\
%A_L \rightarrow - A_L \\$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\hat{e}_B&\hat{e}_C&\cdots&\hat{e}_{K}&\hat{e}_{K+1}&B\\
%	\begin{block}{c[cccccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   	  &\cdots&  0      &   0     &   0     &\cdots&   0        & 1            &{\delta}_1 \\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta_2} + {e}_{K+1}\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots 	  	  &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  	  &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   1  	  &\cdots&0        &   0     &   0     &\cdots& 0          &     0        &{\delta}_{N-M} + {e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots	  &\ddots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  	  &\cdots& 1       &  0      & 0       &\cdots& 0          &  0           &{\delta}_{N-2} + {e}_A\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &  1      &   0     &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_B\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   0     &  1      &\cdots& 0          &     1        & {e}_C - {e}_{K+1}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   1     & 0       &\cdots& -1         &    -1        &{e}_{B} - {e}_{K}\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  1      &\cdots& 0       &    0    &  0      &\cdots& 0          &     0        &{e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots	  &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   1              &  0   	  &\cdots& 1       &    0    &  0      &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_{N-M} \rightarrow A_{N-M} - A_{2N-3-M}  \\
%A_{N-2} \rightarrow A_{N-2} + A_{L}\\
%A_L \rightarrow  A_{N-1} + A_L  \\
%$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\hat{e}_B&\hat{e}_C&\cdots&\hat{e}_{K}&\hat{e}_{K+1}&B\\
%	\begin{block}{c[cccccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   	  &\cdots&  0      &   0     &   0     &\cdots&   0        & 1            &{\delta}_1 \\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta_2} + {e}_{K+1}\\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots 	  	  &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  	  &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   0  	  &\cdots&0        &   0     &   0     &\cdots& 0          &     0        &{\delta}_{N-M} \\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots	  &\ddots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  	  &\cdots& 0       &  1      & 0       &\cdots& 0          &  0           &{\delta}_{N-2} + {e}_B\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 1       &  0      &   0     &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_A\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   0     &  1      &\cdots& 0          &     1        & {e}_C - {e}_{K+1}\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &  -1     & 0       &\cdots&  1         &     1        &{e}_{K} - {e}_B\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  1      &\cdots& 0       &    0    &  0      &\cdots& 0          &     0        &{e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots	  &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   1              &  0   	  &\cdots& 1       &    0    &  0      &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_A\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%On doing the following row transformations,\\ 
%$
%A_{1} \rightarrow A_{1} - A_{N}  \\
%A_{N-2} \rightarrow A_{N-2} + A_{2N-4-M}\\
%A_{N-1} \rightarrow A_{N-1} + A_L\\
%A_L \rightarrow  A_{2N-4-M} + A_L  \\
%A_N \leftrightarrow A_{2N-3-M}\\
%A_L \leftrightarrow A_{2N-4-M}\\
%A_{2N-4-M} \leftrightarrow A_N\\
%$
%the matrix will become \\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccccccccccccccc}
%	ROW       &\hat{\delta}_1&\hat{\delta}_2&\cdots&\hat{\delta}_{N-1-M}&\hat{\delta}_{N-M}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_1&\cdots&\hat{e}_A&\hat{e}_B&\hat{e}_C&\cdots&\hat{e}_{K}&\hat{e}_{K+1}&B\\
%	\begin{block}{c[cccccccccccccccc|c]}
%	A_1       &       1      &      0       &\cdots&     0              &       0          &\cdots&        0         &        0         &  0   	  &\cdots&  0      &   0     &  -1     &\cdots&   0        & 1            &{\delta}_1 - e_C + {e}_{K+1}\\
%	A_2       &      0       &     1        &\cdots&    0               &     0            &\cdots&    0             &      0           &   0     &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta_2} \\
%	\vdots    & \vdots       &     \vdots   &\ddots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\cdots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots 	  	  &\vdots\\
%	A_{N-1-M} &      0       &     0        &\cdots&    1               &     0            &\cdots&    0             &      0           &   0  	  &\cdots& 0       &   0     &   0     &\cdots& 0          &     0  	  &{\delta}_{N-1-M}\\
%	A_{N-M}   &      0       &     0        &\cdots&    0               &     1            &\cdots&    0             &      0           &   0  	  &\cdots&0        &   0     &   0     &\cdots& 0          &     0        &{\delta}_{N-M} \\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\ddots&\vdots            & \vdots           &\vdots	  &\ddots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{N-2}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    1             &      0           &   0  	  &\cdots& 0       &  0      & 0       &\cdots& 1          &  1           &{\delta}_{N-2} + {e}_{K}\\
%	A_{N-1}   &      0       &     0        &\cdots&    0               &     0            &\cdots&    0             &      1           &   0     &\cdots& 0       &  1      &   0     &\cdots& 0          &     0        &{\delta}_{N-1} + {e}_B\\
%	A_{2N-3-M}& 0            &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  1      &\cdots& 0       &    0    &  0      &\cdots& 0          &     0        &{e}_1\\
%	\vdots    & \vdots       &     \vdots   &\cdots& \vdots             & \vdots           &\cdots&\vdots            & \vdots           &\vdots   &\ddots&\vdots   &\cdots   &\cdots   &\vdots&\vdots      &\cdots        &\vdots\\
%	A_{L}     &0             &    0         &\cdots&        0           &     0            &\cdots& 0                &   0              &  0   	  &\cdots& 1       &    0    &  0      &\cdots&-1          &    -1        &{e}_A - e_{K}\\
%	A_{2N-4-M}&0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   1     & 0       &\cdots&  -1        &    -1        &{e}_{B} - {e}_{K}\\
%	A_{N}     &0             &    0         &\cdots&        0           &     0            &\cdots&  0               &   0              &  0      &\cdots& 0       &   0     &  1      &\cdots& 0          &     1        & {e}_C - {e}_{K+1}\\
%	\end{block}
%	\end{blockarray}
%	$\\
%\end{scriptsize}
%From the above matrix structure after row transformations of initial matrix, we can deduce that\\
%rank(A) = rank(A,B) = number of variables  shows that Unique solution is obtained. But this unique solution doesn't find the corresponding counterpart variables and becomes Unique  \& Wrong solution making the system not capable of correcting decoding errors while $K > N-3$ actual errors and $k \leq K$ estimate errors are present on different equations.
%
%Without Loss Of Generality, if $K > N-3$ actual and $k \leq K$ estimate errors are present on different equations, Unique and Wrong Solution can be obtained. Hence, system is not capable of correcting decoding errors if  Unique and Wrong Solution is obtained. 
%
%Hence, an N-node system is not capable of correcting decoding errors for K $\ge$ N-3 actual errors.
%\end{proof}
%For example, Consider a 4-Node system with \textit{K} = 2 $\ge$ 1 [\textit{N-3}]  with $k \le K$, equation system can be represented as,
%
%$
%\hat{\delta}_{01} = \delta_{01} + e_{01} \\
%\hat{\delta}_{02} = \delta_{02} + e_{02}\\
%\hat{\delta}_{03} + \hat{e}_{03} = \delta_{03}\\
%\hat{\delta}_{02} - \hat{\delta}_{01} = \delta_{02} - \delta_{01}\\
%\hat{\delta}_{03} - \hat{\delta}_{01} = \delta_{03} - \delta_{01}\\
%\hat{\delta}_{03} - \hat{\delta}_{02} = \delta_{03} - \delta_{02}\\
%$
%
%Matrix for the above equation system can be written as\\
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{03}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0           &\delta_{01} + {e}_{01}\\
%	A_2       &0                &1                &0                &0           &\delta_{02}+ {e}_{02}\\
%	A_3       &0                &0                &1                &1   		 &\delta_{03}+ {e}_{03} \\
%	A_4       &-1               &1                &0                &0           &\delta_{02} - \delta_{02}\\
%	A_5       &-1               &0                &1                &0           &\delta_{03} - \delta_{01}\\
%	A_6       &0                &-1               &1                &0           &\delta_{03} - \delta_{02}\\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%On doing the following transformations,\\
%$
%A_4 \rightarrow A_4 + A_1\\
%A_5 \rightarrow A_5 + A_1\\
%A_6 \rightarrow A_6 + A_2\\
%$
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{03}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0           &\delta_{01} + {e}_{01}\\
%	A_2       &0                &1                &0                &0           &\delta_{02}+ {e}_{02}\\
%	A_3       &0                &0                &1                &1   		 &\delta_{03}+ {e}_{03} \\
%	A_4       &0                &1                &0                &0           &\delta_{02} + {e}_{01}\\
%	A_5       &0                &0                &1                &0           &\delta_{03} + {e}_{01}\\
%	A_6       &0                &0                &1                &0           &\delta_{03} - \delta_{02}\\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%On doing the following transformations,\\
%$
%A_4 \rightarrow A_4 - A_2\\
%A_5 \rightarrow A_3 - A_5\\
%A_6 \rightarrow A_3 - A_6\\
%$
%\begin{scriptsize}
%	$
%	\begin{blockarray}{cccccc}
%	ROW       &\hat{\delta}_{01}&\hat{\delta}_{02}&\hat{\delta}_{03}&\hat{e}_{03}&B\\
%	\begin{block}{c[cccc|c]}
%	A_1       &1                &0                &0                &0           &\delta_{01} + {e}_{01}\\
%	A_2       &0                &1                &0                &0           &\delta_{02}+ {e}_{02}\\
%	A_3       &0                &0                &1                &1   		 &\delta_{03}+ {e}_{03} \\
%	A_4       &0                &0                &0                &0           &{e}_{01} - e_{02}\\
%	A_5       &0                &0                &0                &1           &e_{14} - {e}_{01}\\
%	A_6       &0                &0                &0                &1           &e_{14} - e_{02}\\
%	\end{block}
%	\end{blockarray}\\
%	$
%\end{scriptsize}
%In the above matrix, rank(A) = rank(A,B) = number of variables confirming Unique but wrong solution as the variables are not yielding their corresponding measured variables as solution making the system  not capable of correcting decoding errors to K\textit{a} = 2 $\ge$ 1 (4-3) actual errors. \\
%
%Hence, an N-node fully connected system can correct a maximum of \textit{N-3} clock-sync errors.
%
%\end{small}
%\twocolumn
%\clearpage

The system of equations represents clock-sync sessions between each pair of nodes in a fully connected system. Hence, total number of equations will be $L$ = \textit{N(N-1)/2}. Out of these equations, \textit{N-1} is the number of Layer-1 equations and the rest are Layer-2 equations. There can be a maximum of \textit{N(N-1)/2} clock-sync errors. If \textit{N-2} number of clock-sync errors are present in the system, say \textit{M} of them are in Layer-1 equations. Here, \{ $\delta_1$,...,$\delta_{N-1}$\} represents \{ $\delta_{ij}$ $|$ $\forall$ i,j $\epsilon$ [0 , N-1], i $\neq$ j \} to make the system more generic so that this equation system can suit \textit{N} number of nodes. This also suits to estimate offset $\hat{\delta}_{ij}$. Errors \{$e_1$,..,$e_{K}$\} represents \{$e_{ij}$ $|$ $\forall$ i,j $\epsilon$ [0 , N-1], i $\neq$ j \} to make the system generic. This also holds for estimate errors $\hat{e}_{ij}$. Given below is the generic structure of equations.\\
%
%
%Generic matrix for above set of equations can be written as 
%$
%\begin{blockarray}{cccccccccccccc}
%ROW    &\hat{\delta}_{1}&\hat{\delta}_{2}&\cdots&\hat{\delta}_{N-2}&\hat{\delta}_{N-1}&\hat{e}_{1}&\cdots&\hat{e}_{M}&\hat{e}_{M+1}&\hat{e}_{M+1}&\cdots&\hat{e}_{K}&B
%\begin{block}{c[cccccccccccc|c]}
%%R_{1,0}  &1 			&0				 &\cdots&0				   &0				  &\hat{a}	  &\cdots&\hat{b}	 &0			   &0		  	 &\cdots&0          &\delta_{10}+ x
%%R_{2,0}  &0 			&1				 &\cdots&0				   &0				  &\cdots	  &\cdots&\cdots	 &\cdots       &\cdots	  	 &\cdots&\cdots     &\delta_{20}+ x
%%\cdots   &\cdots 		&\cdots			 &\ddots&\cdots			   &\cdots			  &\cdots	  &\cdots&\cdots	 &\cdots	   &\cdots		 &\cdots&\cdots		&\cdots
%%R_{N-2,0}&0 			&1				 &\cdots&1				   &0				  &\cdots	  &\cdots&\cdots	 &\cdots       &\cdots	  	 &\cdots&\cdots     &\delta_{\textit{N-2}0}+ x
%%R_{N-1,0}&0 			&0				 &\cdots&0				   &0				  &\cdots	  &\cdots&\cdots	 &\cdots       &\cdots	  	 &\cdots&\cdots     &\delta_{\textit{N-1}0}+ x
%%R_{1,2}  &1				&-1				 &\cdots&0				   &0				  &0		  &\cdots&0		     &c			   &d	         &\cdots&\cdots		&\delta_{10}-\delta_{20}
%%\cdots   &\cdots 		&\cdots			 &\ddots&\cdots			   &\cdots			  &\cdots	  &\cdots&\cdots	 &\cdots	   &\cdots		 &\cdots&\cdots		&\cdots
%%R_{1,N-2}&1				&0				 &\cdots&-1				   &0				  &0		  &\cdots&0		     &\cdots	   &\cdots       &\cdots&\cdots		&\delta_{10}-\delta{\textit{N-2}0}
%%R_{1,N-1}&1				&0				 &\cdots&0				   &-1				  &0		  &\cdots&0		     &c			   &d	         &\cdots&\cdots		&\delta_{10}-\delta{\textit{N-1}0}
%%\cdots   &\cdots 		&\cdots			 &\ddots&\cdots			   &\cdots			  &\cdots	  &\cdots&\cdots	 &\cdots	   &\cdots		 &\cdots&\cdots		&\cdots
%%R_{N-1,N-2}&0				&0				 &\cdots&1				   &-1				  &0		  &\cdots&0		     &c			   &d	         &\cdots&\cdots		&\delta_{10}-\delta{\textit{N-1}0}
%\end{block}
%\end{blockarray}\\
%$
\begin{lemma}
	An N-node system can correct a maximum of N-2 clock-sync errors with N-2 estimates distributed to the equations having ground-truth errors.  
\end{lemma}
\begin{proof}
	
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

